The Self-Replication Phase Diagram: Mapping Where Life Becomes Possible in Cellular Automata Rule Space

What substrate features allow life? We exhaustively classify all 262,144 outer-totalistic binary cellular automata rules with Moore neighbourhood for self-replication and produce phase diagrams in the $(\lambda, F)$ plane, where $\lambda$ is Langton's rule density and $F$ is a background-stability parameter. Of these rules, 20,152 (7.69%) support pattern proliferation, concentrated at low rule density ($\lambda \approx 0.15$--$0.25$) and low-to-moderate background stability ($F \approx 0.2$--$0.3$), in the weakly supercritical regime (Derrida coefficient $\mu = 1.81$ for replicators vs. $1.39$ for non-replicators). Self-replicating rules are more approximately mass-conserving (mass-balance 0.21 vs. 0.34), and this generalises to $k{=}3$ Moore rules. A three-tier detection hierarchy (pattern proliferation, extended-length confirmation, and causal perturbation) yields an estimated 1.56% causal self-replication rate. Self-replication rate increases monotonically with neighbourhood size under equalised detection: von Neumann 4.79%, Moore 7.69%, extended Moore 16.69%. These results identify background stability and approximate mass conservation as the primary axes of the self-replication phase boundary.

==> chapters/03-discussion__Don_Yin_s_conflicted_copy_2026-03-25_.tex <==
\section{Discussion}\label{ch:discussion}

\subsection{Beyond the edge of chaos: conservation as the binding constraint}

The conventional expectation, following \citet{langton1990}, was that self-replication should concentrate at the edge of chaos, where dynamical activity is maximal yet still controllable. Our data refine this picture. Self-replication peaks at $\lambda \approx 0.15$\textendash$0.25$, where the Derrida coefficient is already supercritical: $\mu = 1.81$ for tier-1-positive rules versus $\mu = 1.39$ for tier-1-negative rules at matched $\lambda$. The edge of chaos ($\mu = 1$) itself falls at $\lambda \approx 0.05$\textendash$0.10$, \emph{below} the self-replication peak.

This means self-replicators are not poised at criticality; they inhabit a weakly supercritical regime. Moreover, replicating rules are \emph{more} dynamically active than non-replicating rules at the same $\lambda$, not less. The Derrida gap ($\Delta \mu \approx 0.4$) is consistent with a picture in which replication requires enough perturbation growth to propagate spatial copies, while rules that merely conserve structure without amplifying it cannot sustain proliferation.

If dynamical activity alone were sufficient, the self-replication rate should peak near the Derrida maximum, well above $\lambda = 0.25$. It does not, because a second constraint binds first: approximate mass conservation. Rules at higher $\lambda$ are supercritical but non-conserving; their dynamics destroy patterns faster than copies can form. The binding constraint is therefore conservation, not criticality. Self-replication requires weak supercriticality \emph{plus} approximate conservation, and the narrow $\lambda$ window where both conditions are jointly satisfied defines the island of life in the phase diagram.

This reframes the Langton hypothesis. Dynamical activity at or above the edge of chaos is necessary--- rules in the ordered regime ($\mu < 1$) almost never self-replicate--- but it is not sufficient. Conservation provides the additional structural constraint that channels supercritical dynamics into pattern-preserving replication rather than pattern-destroying chaos.

\subsection{Background stability as a hidden variable}

The adapted $F$ parameter (Section~\ref{ch:methods}; cf.\ \citealp{sakai2004}) captures a dimension of rule structure that $\lambda$ misses: which entries in the rule table are non-quiescent. Two rules with identical $\lambda$ but different $F$ have the same activity level but differ in whether that activity disrupts quiescent regions. Our phase diagrams show that self-replication is localised in the $(\lambda, F)$ plane; background stability is a relevant axis for characterising life-supporting substrates.

\subsection{Approximate conservation without design}

The finding that self-replicating rules are more approximately mass-conserving connects to recent work on mass-conserving \acp{ca}. \citet{plantec2025} showed that adding exact mass conservation to Lenia transforms the system from one where self-maintaining patterns are rare to one where they are abundant. \citet{papadopoulos2025} reported a similar pattern in continuous \acp{ca} using their MaCE framework. Our data extend this pattern to discrete systems: even without explicit conservation constraints, the rules that happen to approximately conserve mass are those most likely to support self-replication. This association survives $\lambda$/$F$ matching (Cohen's $d = -0.94$) and permutation testing ($p < 10^{-4}$).

The conservation effect generalises beyond binary Moore rules. For $k{=}3$ outer-totalistic Moore rules, the mass-balance effect is even stronger ($d = -1.04$, $p = 4.2 \times 10^{-227}$), which suggests that conservation becomes a more powerful discriminator as the state alphabet grows. For the \ac{vn} neighbourhood, the effect is weaker ($d = -0.31$), though this estimate draws on only 49 tier-1-positive rules under the equalised protocol and may be underpowered. Across these three substrates, approximate conservation is a convergent property of life-supporting rules, not merely an engineering convenience imposed by design.

\subsection{Mass-balance as the primary discriminator}

A logistic regression combining $\lambda$, $F$, mass-balance, spatial entropy, and O-information achieves AUC $= 0.85$ for predicting self-replication status, with mass-balance as the dominant feature (standardised coefficient $-2.09$). O-information, despite a significant univariate signal ($d = -0.27$, $p < 10^{-12}$), contributes negligibly once mass-balance is controlled (coefficient $\approx 0$). This indicates that the spatial synergy observed in replicating rules shares substantial variance with approximate conservation: rules that approximately conserve mass tend also to produce synergy-dominated spatial patterns. Conservation, rather than higher-order information structure per se, appears to be the more fundamental substrate property associated with self-replication.

\subsection{Neighbourhood size: monotonically increasing self-replication}

Under an equalised detection protocol--- matching the number of initial conditions and simulation length across neighbourhoods--- self-replication rate increases monotonically with neighbourhood size: \ac{vn} ($|N|{=}5$, 4.79\%) $<$ Moore ($|N|{=}9$, 7.69\%) $<$ extended Moore ($|N|{=}25$, 16.69\%). The original \ac{vn} rate of 33.2\% reflects the higher detection sensitivity of a protocol with $4{\times}$ more initial conditions and $2{\times}$ longer simulation time; once these factors are equalised, the \ac{vn} neighbourhood produces the lowest replication rate, not the highest.

The monotonic relationship admits a straightforward interpretation: larger receptive fields provide each cell with more spatial information for encoding replication mechanisms. A $5 \times 5$ extended Moore kernel can represent spatial templates that are inaccessible to the $3 \times 3$ Moore kernel, which in turn can encode richer neighbour interactions than the 4-cell \ac{vn} kernel. The relationship between neighbourhood size and self-replication is thus governed by information capacity, not by a tension between locality and dilution.

A caveat is warranted: the extended Moore rate (16.69\%) derives from a 10,000-rule sample of the $2^{50}$ rule space, whereas the Moore census is exhaustive. Sampling variance may affect the extended Moore estimate, and the true population rate could differ.

\subsection{Self-replication versus open-endedness}

Comparing our exhaustive self-replication census against \citeauthor{kumar2024}'s (\citeyear{kumar2024}) ASAL open-endedness scores for the same 262,144 rules yields a near-zero correlation ($\rho = -0.002$). CLIP-based visual novelty does not predict self-replication, and self-replicating rules are no more or less ``interesting'' in the ASAL sense than non-replicating rules.

This null result has a clear implication: self-replication is a substrate-structural phenomenon, governed by conservation and mild supercriticality, not by the kind of visual complexity that foundation-model embeddings capture. A rule can produce visually novel, open-ended dynamics without supporting self-replication, and conversely, many self-replicating rules produce visually repetitive patterns that score low on ASAL novelty. The mechanisms that underlie self-replication--- approximate conservation, low $\lambda$, appropriate $F$--- are structural features of the rule table, not emergent aesthetic properties of the dynamics.

\subsection{Comparison with Brown and Sneppen (2025)}

\citet{brown2025} studied replicators in a three-state extension of the Game of Life (``3-Life'') with varying survival thresholds, finding that self-replication emerges preferentially in low-activity regimes. their work, selected as a PRE Editors' Suggestion, provides a deep characterisation of replicator dynamics within a single rule family. our study takes a complementary approach: rather than varying thresholds within one family, we exhaustively survey the full 262,144 outer-totalistic binary rule space and sample 10,000 $k{=}3$ rules, mapping the self-replication phase boundary across substrate parameters. the convergent finding that replication favours low-activity regimes in both studies strengthens confidence that this is a generic property of Life-like substrates, not an artefact of any particular rule family.

our $k{=}3$ sweep (15.55\% tier-1 rate, 95\% CI: [14.85\%, 16.28\%]) provides a quantitative complement to the Brown and Sneppen analysis: by sampling across $k{=}3$ outer-totalistic rule space rather than within a single rule, we can estimate the prevalence of self-replication as a function of $\lambda$ and $F$. the mass-balance finding ($d = -1.04$ for $k{=}3$) suggests that approximate conservation may also be relevant in 3-Life, though \citet{brown2025} did not test this directly. the key difference between the two studies is one of scope versus depth: we provide a systematic phase diagram across substrate parameters, identifying conservation and mild supercriticality as the binding constraints, whereas \citet{brown2025} provide detailed mechanistic analysis of replicator dynamics, including replication cycles and spatial organisation, within a single substrate. the two perspectives are complementary and together suggest that the conditions for self-replication are both narrow and universal across Life-like cellular automata.

\subsection{Limitations}

our pattern-proliferation definition is permissive, but the extended-length rescreen (Section~\ref{sec:tier2}) reproduces 97.8\% of flagged rules, which bounds the non-confirmation rate at 2.2\%. the causal perturbation test (Section~\ref{sec:tier3}) further narrows this to an estimated 1.56\% true causal self-replication rate. of the $n = 978$ confirmed rules tested, the fraction classified as ``robust replicators'' (those that replicate in isolation but tolerate single-cell deletions) may represent a genuine category of robust self-replication or may require multi-cell perturbation tests to reveal fragility. additionally, we tested only outer-totalistic rules. all known non-trivial self-replicators at $k > 2$ use non-totalistic rules with directional information flow \citep{langton1984, hintze2025}. the outer-totalistic restriction may structurally exclude self-replication mechanisms at higher $k$, though our C4 rotationally-symmetric sample (Section~\ref{sec:c4}) begins to probe non-totalistic rule spaces.

the $F$ parameter's axis location in the phase diagram depends on the weighting scheme used to compute it: under alternative weightings the island of life shifts along the $F$ axis, though its existence and localisation are preserved across all weightings tested. this means the precise $F$ coordinates we report are convention-dependent, while the qualitative conclusion--- that background stability is a relevant second axis--- is robust.

the equalised \ac{vn} census reveals that neighbourhood comparisons are sensitive to detection protocol. the raw \ac{vn} rate (33.2\%) and the equalised rate (4.79\%) differ by nearly an order of magnitude, which underscores that protocol-matched comparisons are essential for cross-substrate claims.

\subsection{Outlook}

the immediate next steps are: (1) extending the sweep to $k = 4, 6, 8$ with both outer-totalistic and rotationally-symmetric rules; (2) computing causal emergence \citep{hoel2013} at the phase boundary to test whether the macroscale dynamics of self-replicating rules carry more effective information than their microscale; (3) extending the Derrida analysis to continuous \ac{ca} substrates (Lenia, Flow-Lenia) to test whether the weakly supercritical regime generalises beyond discrete systems; and (4) investigating why the mass-balance effect is weaker for \ac{vn} than for Moore and $k{=}3$--- whether this reflects a genuine substrate difference or merely the small sample size under equalised detection.

